KRATTA, a versatile triple telescope array for charged reaction products

A new detection system KRATTA, Krak\'ow Triple Telescope Array, is presented. This versatile, low threshold, broad energy range system has been built to measure the energy, emission angle, and isotopic composition of light charged reaction products. It consists of 38 independent modules which can be arranged in an arbitrary configuration. A single module, covering actively about 4.5 msr of the solid angle at the optimal distance of 40 cm from the target, consists of three identical, 0.500 mm thick, large area photodiodes, used also for direct detection, and of two CsI(1500 ppm Tl) crystals of 2.5 and 12.5 cm length, respectively. All the signals are digitally processed. The lower identification threshold, due to the thickness of the first photodiode, has been reduced to about 2.5 MeV for protons (~0.065 mm of Si equivalent) by applying a pulse shape analysis. The pulse shape analysis allowed also to decompose the complex signals from the middle photodiode into their ionization and scintillation components and to obtain a satisfactory isotopic resolution with a single readout channel. The upper energy limit for protons is about 260 MeV. The whole setup is easily portable. It performed very well during the ASY-EOS experiment, conducted in May 2011 at GSI. The structure and performance of the array are described using the results of Au+Au collisions at 400 MeV/nucleon obtained in this experiment.

==> PaxHeaders.25986/lukasik_arxiv.tex <==
30 mtime=1357825341.399439838
30 atime=1357825370.168440417
30 ctime=1357825341.399439838

